Local Enumeration and Majority Lower Bounds

Depth-3 circuit lower bounds and $k$-SAT algorithms are intimately related; the state-of-the-art $\Sigma^k_3$-circuit lower bound and the $k$-SAT algorithm are based on the same combinatorial theorem. In this paper we define a problem which reveals new interactions between the two. Define Enum($k$, $t$) problem as: given an $n$-variable $k$-CNF and an initial assignment $\alpha$, output all satisfying assignments at Hamming distance $t$ from $\alpha$, assuming that there are no satisfying assignments of Hamming distance less than $t$ from $\alpha$. Observe that: an upper bound $b(n, k, t)$ on the complexity of Enum($k$, $t$) implies: - Depth-3 circuits: Any $\Sigma^k_3$ circuit computing the Majority function has size at least $\binom{n}{\frac{n}{2}}/b(n, k, \frac{n}{2})$. - $k$-SAT: There exists an algorithm solving $k$-SAT in time $O(\sum_{t = 1}^{n/2}b(n, k, t))$. A simple construction shows that $b(n, k, \frac{n}{2}) \ge 2^{(1 - O(\log(k)/k))n}$. Thus, matching upper bounds would imply a $\Sigma^k_3$-circuit lower bound of $2^{\Omega(\log(k)n/k)}$ and a $k$-SAT upper bound of $2^{(1 - \Omega(\log(k)/k))n}$. The former yields an unrestricted depth-3 lower bound of $2^{\omega(\sqrt{n})}$ solving a long standing open problem, and the latter breaks the Super Strong Exponential Time Hypothesis. In this paper, we propose a randomized algorithm for Enum($k$, $t$) and introduce new ideas to analyze it. We demonstrate the power of our ideas by considering the first non-trivial instance of the problem, i.e., Enum($3$, $\frac{n}{2}$). We show that the expected running time of our algorithm is $1.598^n$, substantially improving on the trivial bound of $3^{n/2} \simeq 1.732^n$. This already improves $\Sigma^3_3$ lower bounds for Majority function to $1.251^n$. The previous bound was $1.154^n$ which follows from the work of H{\aa}stad, Jukna, and Pudl\'ak (Comput. Complex.'95).

==> sections/algorithm.tex <==
% !TEX root = ../paper.tex
\section{Algorithm for $\enumballsat{k}{t}$} \label{sec:algorithm}

\RestyleAlgo{ruled}

\begin{algorithm}
\caption{Local Enumeration Algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$k$-CNF $F = (X, \cC)$, distance $r$}
\SetKwFunction{FRecurseInBall}{Recursive Local Enumeration}
\label{algo:local-enumeration}
Let $S$ be the maximal set of disjoint monotone clauses in $F$.\\
Let $O$ be the list of the clauses starting with the clauses in $S$ followed by the rest of the clauses in some arbitrary but fixed order.\\
Return \FRecurseInBall($F, r, O$)\\
\vspace{0.75\baselineskip}

\FRecurseInBall{$F, r, O$} {\\
\eIf{$O$ contains an  empty clause} {
    \Return{Empty list}
}
{\eIf{$r=0$} {
    \eIf{$\cC$ does not contain a monotone clause}{
    \Return{List containing the  all-$0$ assignment}
    }
    {
    \Return{Empty list}
    }
   }
  {\eIf{$O$ is non empty}{
    Let $C$ be the first entry of $O$.\\
    %Let $O'$ be the list $O$ with the first entry removed.
%}
%{
    %Let $C$ be arbitrary monotone clause from $\cC$.\\
    %Let $O'$ be $O$.\\
%}
    Let $(v_1, v_2, \dots, v_w)$ be a random permutation of the variables in the monotone clause $C$.\\
    Let $L$ be an empty list.\\
    \For{$i\leftarrow 1$ \KwTo $w$}{
         $F_i\gets$ the formula obtained by setting the variables $v_1, \dots, v_{i-1}$ to $0$ and $v_i$ to $1$ in $F$.\\
         Let $L_i$ be the list returned by \FRecurseInBall($F_i, r-1, O'$)\\
         \For{every assignment $\alpha$ in $L_i$}{
             Let $\beta$ be the assigment obtained by setting variables $v_1, \dots, v_{i-1}$ to $0$, setting variable $v_i$ to $1$, and the remaining variables according to $\alpha$.\\
             Add $\beta$ to list $L$.
         }
    }
    \Return{List $L$}\\
}
{
\Return{Empty list}
}
}
}
}
\end{algorithm}


Let $F = (X, \cC)$ be a $k$-CNF with variable set $X$ 
and clause set $\cC$. 
Let $r\in [n]$ and $c\in \zo^n$ be such 
that every satisfying assignment of $F$ is at a distance
of at least $r$ from $c$. We will describe a local 
enumeration procedure that will output all satisfying assignments at distance exactly 
$r$ from $c$. Notice that this suffices to solve \enumballsat{k}{t} as 
we can run this procedure for each setting of $r = 1, 2, \dots, t$ until 
we hit a value of $r$ where we do find satisfying assignments. 
As mentioned earlier, our local enumeration algorithm can be thought of as a randomized Monien-Speckenmeyer algorithm. 

Without loss of generality, assume that
$c = 0^n$. Indeed, let $G$ be the $k$-CNF formula over 
the variable set $X$. $G$'s clause set is obtained from that of
$F$ by the following replacement of literals:  
For each variable $v\in X$, if $c$ sets $v$ to $1$, 
then we swap occurrences of the positive and the negative 
literals corresponding to $v$ in $\cC$. 
Otherwise, if $c$ sets $v$ to $0$,  we leave the corresponding literals
as they are.
$G$ is also a $k$-CNF formula and for all $y\in \zo^n$, $G(y) = F(y\oplus c)$. Clearly, there exists a satisfying assignment within distance $r$ 
from $0^n$ in $G$ if and only if there exists a satisfying assignment 
within distance $r$ from $c$ in $F$. 
%We observe the following:

%\begin{observation}
%For a $k$-CNF formula $F$, either $0^n$ is a satisfiable assignment or there exists a positive monotone clause in $F$.
%\end{observation}


For our local enumeration algorithm, if the $r=0$, then we easily 
check whether $0^n$ is a satisfying assignment and output it if it is. 
Otherwise, there must always exist a positive monotone clause in $F$. 
We fix such a monotone clause and let
$v_1, \dots, v_k$
be its variables after a random ordering.
Let $F_1, \dots, F_k$ be $k$-CNFs where $F_i$ is obtained by setting $v_i$ to $1$ and $v_1, \dots, v_{i-1}$ to $0$. We then recursively enumerate all satisfying assignments at distance $r-1$ 
from $0^{n-i}$ in each $F_i$ (over $n-i$ variables). 
The following observation makes it clear
that \cref{algo:local-enumeration} 
indeed enumerates all satisfying assingments at distance 
$r$ from $0^n$ (regardless of the random choices). 
%We observe the following regarding these $F_i$:

\begin{observation}
Let $\alpha$ be a satisfying assignment of $F_i$ at distance $r-1$ from $0^n$. Then, $\alpha$ is in 1-1 correspondence with a satisfying assignment $\beta$ of $F$ that is at distance $r$ from $0^n$. This correspondence is given by letting $\beta$ be the assignment obtained by setting variables in $X\setminus \{v_1, \dots, v_i\}$ according to $\alpha$ and setting $v_1 = \dots = v_{i-1} = 0, v_i = 1$.
\end{observation}

The expected runtime of this algorithm is much less clear. Our
main result \cref{thm:main-result} provides an analysis of the 
algorithm. For this purpose, we define the notion of 
a \emph{transversal tree} where each satisfying assignment
at distance $r$ from $0^n$ appears as a leaf. Thus the size of the
transversal tree is an upper bound on the running time
of the algorithm. which might also be of independent interest. 
We first bound the size of the size of the transversal tree for the monotone case and extend it to the non-monotone case.
These bounds are presented in 
\cref{sec:monotone}  and
\cref{sec:non-monotone}. 
%Translating into that language, 
%\cref{algo:local-enumeration} actually 
%produces a transversal tree and we bound the size of that transversal tree.

The maximal set $S$  of disjoint monotone clauses 
appearing at the beginning of the list $O$ guarantees
that the first the first $|S|$ levels of the transversal tree constructed by the algorithm involves the same monotone clause.
%that appear 
%hat by fixing a maximal
%that \cref{algo:local-enumeration} actually fixes 
%a maximal set of disjoint monotone clauses and ensures the same monotone disjoint clause is chosen across various branches of the algorithm. 
This simplifies the analysis of the algorithm and probably produces a better bound.
%This does not affect the correctness of the procedure and this is done only to improve the expected runtime of the algorithm and so that its easier to analyze the resultant transversal tree.




% \begin{algorithm}
% \caption{Recursive Local Enumeration function}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{A $k$-CNF $F = (X, \cC)$, radius $r$, an ordering of some clauses $O$}
% \If{$r < 0$} {
%     \Return{False}
% }
% \If{$\cC$ does not contain a monotone clause}{
%     \Return{True}
% }
% \eIf{$O$ is non empty}{
%     $C\gets O[0]$\\
%     $O'\gets O[1:]$\\
% }
% {
%     $C\gets $ arbitrary monotone clause from $\cC$.\\
%     $O'\gets O$.\\
% }
% Let $(v_1, v_2, \dots, v_w)$ be a random permutation of the variables in the monotone clause $C$.\\
% \For{$i\leftarrow 1$ \KwTo $w$}{
%     $F'\gets$ the simplified formula obtained by setting the variables $v_1, \dots, v_{i-1}$ to $0$ and $v_i$ to $1$ in $F$.
%     \If{SearchInBallRecursive($F', r-1, O'$) returns True} {
%         \Return{True}
%     }
% }
% \Return{False}
% \end{algorithm}












==> sections/prop.tex <==

We will first establish a recurrence for $M(w, d)$:

\begin{proposition}
\label{claim:Mwd-recurrence}
For $0\le w\le 3d$ and $d\le n$, $M(w, d)$ satisfies the following recurrence:
\begin{align*}
M(w, d) 
\begin{cases}
 = 1 &\text{for $d=0$}\\
 = 3^d &\text{for $w=0$}\\
 = \frac{5}{6}3^d &\text{for $w=1, d\geq 1$}\\
 \leq  (\frac{5}{6})^2 3^d &\text{for $w=2, d\geq 1$}\\
\end{cases}\\
\end{align*}
\begin{align*}
M(w, d) 
\le   \max
\begin{cases}
3M(w, d-1)\\
%&\textrm{if the root node has no marked child edges}  \\
(2+\lambda)M(w-1, d-1) \\
%&\textrm{if the root node has one marked child edge}  \\
(1+2\lambda)M(w-2, d-1), 3\lambda \\
%&\textrm{if the root node has two marked child edges}  \\
M(w-3, d-1) \\
%&\textrm{if the root node has three marked child edges}  \\
\end{cases}
& \text{for $w\geq 3, d\geq 1$}
\end{align*}
\end{proposition}

\begin{proof}
Let $T_u$ be  subtree of $T$ of depth $d$ with root $u$
where every root to leaf shoot has an extended weight of at least $w$.
The base cases can be verified directly. Assume that $d\geq 1$ and $w\geq 3$.
Let $l$ be the number of marked child edges for $u$.
Since $F$ is a $3$-CNF, $l\in\{0,1,2,3\}$.
For each value of $l$,
we use \cref{path-pessim} to bound the value of $M(w,d)$ recursively.
\end{proof}


==> sections/temp.tex <==
\subsubsection{Proof of \cref{thm:Mwd}}
Let $T'$ be a tree of depth $d$ and let every shoot $S_{rv}$
from root $r$ to leaf $v$ of $T'$ has weight at least $0\leq w\leq 3d$.
It is clear that the survival probability $\total'(T')$ is determined once
the edges are marked consistent with the fact that every shoot has weight at least $w$.
We say that a tree $T$ of depth $d$ and weight $w$
is \emph{normal} if it has the following marking:
Let $w=id+j$ where $0\leq i\leq 3$ and $0\leq j<d$.
Nodes in the tree are stratified into $d$ levels where the root is at level $0$
and the leaves at depth $d$ are at level $d$.
Mark $i+1$ children of every non-leaf node at the 
first $j-1$ levels if $j\geq 1$ and mark $i$ children
for each of the remaining non-leaf nodes.
We will show that normal tree maximize has the largest
survival probability by induction on $d$.

Let $T''$ be a tree of depth $w$ and weight $w$ of maximum survival probability.
Assume that $T''$ is not normal.
Let $r$ be the root of $T''$. Assume $l_1$ of the children of $r$ are marked.
Let $T''_1, T''_2, T''_3$ be subtrees of of $T''$ of depth $d-1$ 
and weight $w-i$ with $r_1, r_2, r_3$ as their root nodes respectively.
They are normal and identical by induction hypothesis.
Assume that $l_2$ child edges of each of $r_i$ are marked.
The survival probability of $T''$ is 
$(3-l_1 +l_1 \lambda)(3-l_2 - l_2\lambda)X$.
We argue that the $M'(w,d) = \total'(T')$.




==> sections/turan.tex <==
% !TEX root = ../paper.tex
\section{Tur{\'a}n's theorem (under construction)} \label{sec:turan}

Define $f(n, t)$ to be the minimum $w$ such that every $n$-vertex graph with transversal number at least $t$ has a transversal tree with weight at most $w$. We will show that $f(n, n - 2) \le n^2/4 + O(n \log n)$.

\begin{lemma}
Let $G = (V, E)$ be a graph with transversal number at least $t$ and let $v \in V$. There exists a transveral tree for $G$ such that the sum of weights of all root to leaf path which include $v$ is at most $f(n - 1, t - 1)$.
\end{lemma} 

\begin{proof}
Let $T$ be a transversal tree of weight $f(n - 1, t - 1)$ for $G - v$. Since $G$ has transversal number at least $t$, no leaf in $T$ can be a transversal for $G$ and therefore for each leaf there is at least one edge which is not covered. We can therefore extend the tree by such an edge and obtain a transversal tree $T'$ of depth $t$ for $G$. Consider a root to leaf path in $T'$ consisting of $v$. Since $v$ can only appear as the last label and hence unmarked, the survival probabiliy of this path is exactly the same as the survival probabiliy of the corresponding path in $T$. Summing over all such paths and since no path in $T$ is counted more than once we get the lemma.
\end{proof}


